Do LLMs Really Adapt to Domains? An Ontology Learning Perspective

Large Language Models (LLMs) have demonstrated unprecedented prowess across various natural language processing tasks in various application domains. Recent studies show that LLMs can be leveraged to perform lexical semantic tasks, such as Knowledge Base Completion (KBC) or Ontology Learning (OL). However, it has not effectively been verified whether their success is due to their ability to reason over unstructured or semi-structured data, or their effective learning of linguistic patterns and senses alone. This unresolved question is particularly crucial when dealing with domain-specific data, where the lexical senses and their meaning can completely differ from what a LLM has learned during its training stage. This paper investigates the following question: Do LLMs really adapt to domains and remain consistent in the extraction of structured knowledge, or do they only learn lexical senses instead of reasoning? To answer this question and, we devise a controlled experiment setup that uses WordNet to synthesize parallel corpora, with English and gibberish terms. We examine the differences in the outputs of LLMs for each corpus in two OL tasks: relation extraction and taxonomy discovery. Empirical results show that, while adapting to the gibberish corpora, off-the-shelf LLMs do not consistently reason over semantic relationships between concepts, and instead leverage senses and their frame. However, fine-tuning improves the performance of LLMs on lexical semantic tasks even when the domain-specific terms are arbitrary and unseen during pre-training, hinting at the applicability of pre-trained LLMs for OL.

==> sections/code/prompts.tex <==
\begin{lstlisting}[caption=Prompts for each model/task pair.]
# GPT3.5
The input data contains a concept, its part-of-speech tagging and its definition. It is expected that you may not know some of those words.
Extract a taxonomy of ALL the terms used in the definition, and only those terms (including the defined concept). Only use the relations: "is a subclass" of and "is a component of" .
Your response should only contain a JSON object, AND NO OTHER TEXT. The format is:
```json
{
    "thoughts": "Reason step by step and write your justifications here.",
    "triples" : [
        {"subject" : "subclass", "predicate": "is a subclass of", "object": "superclass"},
        {"subject" : "part", "predicate": "is a component of", "object": "whole"}
    ]
}
```

Example query:

Concept name: carrot juice
Part-of-speech: noun
Definition: Juice made out of carrot

Expected answer (with NOTHING ELSE):
```json
{
    "thoughts": "The definition states that 'carrot juice' is a 'juice', hence 'carrot juice' is a subclass of 'juice'. Moreover, the definition mentions that 'carrot juice' is made from 'carrot', hence 'carrot' is a component of 'carrot juice'.",
    "triples": [
        {"subject" : "carrot juice", "predicate": "is a subclass of", "object": "juice"},
        {"subject" : "carrot", "predicate": "is a component of", "object": "carrot juice"}
    ]
}
```

INPUT DATA :
Concept name: confectionery
Part-of-speech: noun
Definition: candy and other sweets considered collectively


# LLaMa 2

% TODO: Add the prompt here.

# Zephyr

% TODO: Add the prompt here.


\end{lstlisting}\label{prompts}

RELATION EXTRACTION

GPT 3.5

The input data contains a concept, its part-of-speech tagging and its definition. It is expected that you may not know some of those words.
Extract a taxonomy of ALL the terms used in the definition, and only those terms (including the defined concept). Only use the relations: "is a subclass" of and "is a component of" .
Your response should only contain a JSON object, AND NO OTHER TEXT. The format is:

```json
{
    "thoughts": "Reason step by step and write your justifications here.",
    "triples" : [
        {"subject" : "subclass", "predicate": "is a subclass of", "object": "superclass"},
        {"subject" : "part", "predicate": "is a component of", "object": "whole"}
    ]
}
```

Example query:

Concept name: carrot juice
Part-of-speech: noun
Definition: Juice made out of carrot

Expected answer (with NOTHING ELSE):
```json
{
    "thoughts": "The definition states that 'carrot juice' is a 'juice', hence 'carrot juice' is a subclass of 'juice'. Moreover, the definition mentions that 'carrot juice' is made from 'carrot', hence 'carrot' is a component of 'carrot juice'.",
    "triples": [
        {"subject" : "carrot juice", "predicate": "is a subclass of", "object": "juice"},
        {"subject" : "carrot", "predicate": "is a component of", "object": "carrot juice"}
    ]
}
```

INPUT DATA :
Concept name: {writtenRep}
Part-of-speech: {pos}
Definition: {definition}

LLAMA

The input data contains a concept, its part-of-speech tagging and its definition. It is expected that you may not know some of those words.
Extract a taxonomy of ALL the terms used in the definition, and only those terms (including the defined concept). Only use the relations: "is a subclass" of and "is a component of" .
Your response should only contain a JSON object, AND NO OTHER TEXT. The format is:

```json
{
    "thoughts": "Reason step by step and write your justifications here.",
    "triples" : [
        {"subject" : "subclass", "predicate": "is a subclass of", "object": "superclass"},
        {"subject" : "part", "predicate": "is a component of", "object": "whole"}
    ]
}
```

Example query:

Concept name: carrot juice
Part-of-speech: noun
Definition: Juice made out of carrot

Expected answer:
```json
{
    "thoughts": "The definition states that 'carrot juice' is a 'juice', hence 'carrot juice' is a subclass of 'juice'. Moreover, the definition mentions that 'carrot juice' is made from 'carrot', hence 'carrot' is a component of 'carrot juice'.",
    "triples": [
        {"subject" : "carrot juice", "predicate": "is a subclass of", "object": "juice"},
        {"subject" : "carrot", "predicate": "is a component of", "object": "carrot juice"}
    ]
}
```

INPUT DATA :
Concept name: {writtenRep}
Part-of-speech: {pos}
Definition: {definition}


ZEPHYR

Extract a taxonomy of ALL the terms used in the definition, and only those terms (including the defined concept). Only use the relations: "is a subclass" of and "is a component of" .
Your response should only contain a JSON object, AND NO OTHER TEXT. The format is:

```json
{
    "thoughts": "Reason step by step and write a concise justification here.",
    "triples" : [
        {"object" : "subclass", "predicate": "is a subclass of", "object": "superclass"},
        {"subject" : "part", "predicate": "is a component of", "object": "whole"}
    ]
}
```

Example query:

Concept name: carrot juice
Part-of-speech: noun
Definition: Juice made out of carrot

Expected answer:
```json
{
    "thoughts": "The definition states that 'carrot juice' is a 'juice', hence 'carrot juice' is a subclass of 'juice'. Moreover, the definition mentions that 'carrot juice' is made from 'carrot', hence 'carrot' is a component of 'carrot juice'.",
    "triples": [
        {"subject" : "carrot juice", "predicate": "is a subclass of", "object": "juice"},
        {"subject" : "carrot", "predicate": "is a component of", "object": "carrot juice"}
    ]
}
```

Query:

Concept name: {writtenRep}
Part-of-speech: {pos}
Definition: {definition}

TAXONOMY DISCOVERY

LLAMA
Identify whether CONCEPT A is a subclass of CONCEPT B.
Your response should only contain one single JSON object, AND NOTHING ELSE. You must use the following format:
```json
{
    "thoughts": "Reason step by step and write your justifications in one line here. This string can be empty.",
    "answer": true or false, but not both
}
```

Example query:

CONCEPT A: potato
Definition: an edible tuber native to South America; a staple food of Ireland

CONCEPT B: root vegetable
Definition: any of various fleshy edible underground roots or tubers

Expected answer:
```json
{
    "thoughts": "a potato is an edible tuber, which fits the definition of root vegetable.",
    "answer": true
}
```

Query:

CONCEPT A: {writtenRep_a}
Definition: {definition_a}

CONCEPT B: {writtenRep_b}
Definition: {definition_b}


ZEPHYR

Identify whether CONCEPT A is a subclass of CONCEPT B.
Your response should only contain one single JSON object, AND NOTHING ELSE. You must use the following format:

```json
{
    "thoughts": "Reason step by step and write your justifications in one line here. This string can be empty.",
    "answer": true or false, but not both
}
```

Example query:

CONCEPT A: potato
Definition: an edible tuber native to South America; a staple food of Ireland

CONCEPT B: root vegetable
Definition: any of various fleshy edible underground roots or tubers

Expected answer:
```json
{
    "thoughts": "a potato is an edible tuber, which fits the definition of root vegetable.",
    "answer": true
}
```

Query:

CONCEPT A: {writtenRep_a}
Definition: {definition_a}

CONCEPT B: {writtenRep_b}
Definition: {definition_b}

==> sections/code/rules.tex <==
\begin{lstlisting}[caption=Trimmed Datalog rules and prefixes.]
PREFIX gwn: <https://globalwordnet.github.io/schemas/wn#>
PREFIX ontolex: <http://www.w3.org/ns/lemon/ontolex#>
PREFIX rdf: <http://www.w3.org/1999/02/22-rdf-syntax-ns#>
PREFIX sct: <http://shortcut.org/terms/>

# Written forms  and Definitions of Lexical Concepts
[?i, sct:writtenForm, ?f] :- [?i, rdf:type, ontolex:LexicalConcept], [?s, ontolex:isLexicalizedSenseOf, ?i], [?e, ontolex:sense, ?s], [?e, ontolex:canonicalForm, ?g], [?g, ontolex:writtenRep, ?f].
[?i, sct:definition, ?d] :- [?i, gwn:definition, ?b], [?b, rdf:value, ?d].
[?s, sct:writtenForm, ?f] :- [?s, rdf:type, ontolex:LexicalSense], [?e, ontolex:sense, ?s], [?e, ontolex:canonicalForm, ?g], [?g, ontolex:writtenRep, ?f].

# Hypernymy transitivity
[?s, sct:hypernym, ?o] :- [?s, gwn:hypernym, ?o].
[?s, sct:hypernym, ?o] :- [?s, sct:hypernym, ?a], [?a, sct:hypernym, ?o].
[?s, sct:hyponym, ?o] :- [?s, gwn:hyponym, ?o].
[?s, sct:hyponym, ?o] :- [?s, sct:hyponym, ?a], [?a, sct:hyponym, ?o].

# Derivation between two concepts
[?s, sct:derivation, ?t] :- [?a, ontolex:isLexicalizedSenseOf, ?s], [?a, gwn:derivation, ?b], [?b, ontolex:isLexicalizedSenseOf, ?t].
\end{lstlisting}\label{rules_sct}

==> sections/experiments.tex <==
\section{Experiments}

In this section, we explore the off-the-shelf evaluation proposed in Subsection~\ref{evaluation_protocol}, and the fine-tuning experiments described in Subsection~\ref{finetuning_protocol}.

\subsection{Experimental setup}

\subsubsection{Datasets.} To assess the performance variation with domain specificity, we generate three synthetic domain-specific datasets as parallel corpora from the Open English WordNet~\cite{oewn}, using the methodology described in Section~\ref{gibberish_dataset}. They are:
\begin{itemize}
    \item Sweets: A collection of concepts related to sweets, desserts, sweet food or sugar. In this dataset, hypernyms are frequent, and concepts are relatively well constructed from their hypernyms.
    \item Football: A collection of concepts related to football. This dataset, created by browsing co-topic concepts, includes fewer taxonomic relationships, but has its own terminology and jargon.
    \item Music: A collection of concepts related to musical instruments. It is the largest of the three.
\end{itemize}
Table~\ref{tab:statistics} shows, for each dataset, the number of concepts, the number of hypernymy relationships, the exploration depth and the root concepts. The translator $T$ used to generate gibberish representations of concepts is available online.\footnote{\url{https://github.com/htmai-880/gibberify}}

\begin{table}[t]
\centering
\caption{Dataset statistics. The `Hypernyms' column indicates the number of retrieved hypernymy relationships within the dataset. The `Depth' column indicates the exploration depth of the algorithm.}
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccc}
\toprule
\multirow{2}{*}{$\mathcal{D}$} & \multirow{2}{*}{\textbf{Concepts}} & \multirow{2}{*}{\textbf{Hypernyms}} & \multirow{2}{*}{\textbf{Depth}} & \multirow{2}{*}{\textbf{Root Concepts}} \\
 & & & & \\
\midrule
\textbf{WN-sweets} & 244 & 418 & 5 & sweet (n), sweet (a), sugar\\
\textbf{WN-football} & 937 & 1401 & 5 & football, team, offensive (a), defensive (a) \\
\textbf{WN-music} & 1366 & 2497 & 5 & musical instrument \\
\bottomrule
\end{tabular}
}
\label{tab:statistics}
\end{table}

\subsubsection{Models.}
While this study is not comprehensive of all existing LLMs, our goal is to show a particular trend between them. In the off-the-shelf evaluation, we evaluate the following popular LLMs, with their number of parameters between parentheses: GPT-3.5~\cite{brown2020language} (174B), GPT-4~\cite{openai2024gpt4} ($\geq$ 1T), LLaMa2-13B~\cite{touvron2023llama} (13B), and Zephyr-7B-$\beta$~\cite{tunstall2023zephyr} (7B). The former two, managed by OpenAI and managed by OpenAI and accessed with a paid subscription, are closed-source, whereas the latter two are open-source. In the fine-tuning experiment, we consider Zephyr-7B-$\beta$~\cite{tunstall2023zephyr} and Falcon-7B~\cite{falcon40b}, which are both open-source. We limit our budget to 15\euro{} per dataset.

\subsubsection{Specificities.} We henceforth consider the three following evaluation methods:
\begin{itemize}
    \item Ground-truth (GT)(\texttt{en}) vs \texttt{en}  we compare the answers on the original English dataset against the ground-truth
    \item Ground-truth (GT)(\texttt{gib}) vs \texttt{gib}: we compare the answers on the gibberish dataset against the gibberish ground-truth
    \item \texttt{en} vs \texttt{gib}: using the answers on the original dataset as a ground-truth, we evaluate the consistency of the predictions on the gibberish dataset, regardless of their correctness.
\end{itemize}
In the relation extraction (GT(X) vs X), due to the scarcely annotated holonymy relationships in WordNet, we focus on hypernymy relationships to compute metrics. Moreover, a model prediction is processed by taking into account the inferred hypernymy relationships, using the transitive property of the relation. For instance, if a model outputs the triples (vanilla pudding, is a subclass of, custard-like pudding), and (custard-like pudding, is a subclass of, pudding), we count the triple (vanilla pudding, is a subclass of, pudding) as effectively predicted by the model. In the taxonomy discovery task, predictions that are neither ``True" or ``False" are ignored. Thus, macro-averaged F1-scores may not be between the macro-averaged precisions and the macro-averaged recalls.

\subsection{Off-the-Shelf Evaluation}

\subsubsection{Metrics.} For each model/task configuration, we compute metrics in three settings: GT(\texttt{en}) vs \texttt{en}, GT(\texttt{gib}) vs \texttt{gib}, and \texttt{en} vs \texttt{gib}. The goal is to see if the predictions with gibberish terms align with the predictions with the real terms. We compute the following metrics: precision, recall and F1-score.

\begin{table}[t]
    \centering
    \caption{Results on the relation extraction task in the GT(X) vs X setting, where X is either \texttt{en} or \texttt{gib}. Only hypernymy relations are considered.}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cp{1.cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}}
    \toprule
         \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{X}} & \multicolumn{3}{c}{\textbf{WN-sweets}} & \multicolumn{3}{c}{\textbf{WN-football}} & \multicolumn{3}{c}{\textbf{WN-music}}  \\
         \cline{3-11}
         & & Pre. & Rec. & F1 & Pre. & Rec. & F1 & Pre. & Rec. & F1\\
    \midrule
    \multirow{2}{*}{GPT-3.5} & \texttt{en} & 0.478 & 0.150 & 0.228 & 0.383 & 0.056 & 0.097 & 0.397 & 0.060 & 0.104 \\
         & \texttt{gib} & 0.336 & 0.069 & 0.115 & 0.371 & 0.035 & 0.065
         & 0.307 & 0.029 & 0.053 \\
         \midrule
    \multirow{2}{*}{GPT-4} & \texttt{en} & 0.583 & 0.160 & 0.251 & - & - & - & - & - & - \\
         & \texttt{gib} & 0.530 & 0.129 & 0.207 & - & - & - & - & - & - \\
         \midrule
    \multirow{2}{*}{LLaMa2-13B} & \texttt{en} & 0.536 & 0.141 & 0.223 & 0.423 & 0.035 & 0.065 & 0.434 & 0.030 & 0.056 \\
         & \texttt{gib} & 0.365 & 0.085 & 0.138 & 0.341 & 0.018 & 0.035 & 0.296 & 0.014 & 0.026 \\
         \midrule
    \multirow{2}{*}{Zephyr-7B-$\beta$} & \texttt{en} & 0.441 & 0.158 & 0.233 & 0.399 & 0.067 & 0.115 & 0.374 & 0.063 & 0.108 \\
         & \texttt{gib} & 0.243 & 0.095 & 0.137 & 0.313 & 0.052 & 0.089 & 0.261 & 0.044 & 0.075 \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:gt_rel_extraction_results}
\end{table}

\begin{table}[t]
    \centering
        \caption{Results (macro-average) on the taxonomy discovery task in the GT(X) vs X setting, where X is either \texttt{en} or \texttt{gib}.}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cp{1.cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}}
    \toprule
         \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{X}} & \multicolumn{3}{c}{\textbf{WN-sweets}} & \multicolumn{3}{c}{\textbf{WN-football}} & \multicolumn{3}{c}{\textbf{WN-music}}  \\
         \cline{3-11}
         & & Pre. & Rec. & F1 & Pre. & Rec. & F1 & Pre. & Rec. & F1\\
    \midrule
    \multirow{2}{*}{GPT-3.5} & \texttt{en} & 0.944 & 0.937 & 0.940 & 0.758 & 0.701 & 0.648 & 0.829 & 0.858 & 0.818 \\
         & \texttt{gib} & 0.783 & 0.539 & 0.446 & 0.640 & 0.505 & 0.333 & 0.687 & 0.537 & 0.361 \\
         \midrule
    \multirow{2}{*}{GPT-4} & \texttt{en} & 0.949 & 0.943 & 0.945 & - & - & - & - & - & - \\
         & \texttt{gib} & 0.591 & 0.576 & 0.566 & - & - & - & - & - & - \\
         \midrule
    \multirow{2}{*}{LLaMa2-13B} & \texttt{en} & 0.819 & 0.772 & 0.750 & 0.808 & 0.811 & 0.809 & 0.785 & 0.800 & 0.790 \\
         & \texttt{gib} & 0.450 & 0.447 & 0.444 & 0.533 & 0.531 & 0.504 & 0.576 & 0.556 & 0.465 \\
         \midrule
    \multirow{2}{*}{Zephyr-7B-$\beta$} & \texttt{en} & 0.899 & 0.897 & 0.898 & 0.813 & 0.751 & 0.759 & 0.821 & 0.762 & 0.778 \\
         & \texttt{gib} & 0.691 & 0.634 & 0.621 & 0.500 & 0.500 & 0.469 & 0.530 & 0.524 & 0.523 \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:gt_tax_disc_results}
\end{table}

\begin{table}[t]
    \centering
        \caption{Alignment results (macro-average) on the relation extraction task in the \texttt{en} vs \texttt{gib} setting. Both hypernymy and holonymy relations are considered.}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cp{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}}
    \toprule
         \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{WN-sweets}} & \multicolumn{3}{c}{\textbf{WN-football}} & \multicolumn{3}{c}{\textbf{WN-music}}  \\
         \cline{2-10}
         & Pre. & Rec. & F1 & Pre. & Rec. & F1 & Pre. & Rec. & F1\\
    \midrule
    \multirow{1}{*}{GPT-3.5}  & 0.371 & 0.304 & 0.334 & 0.263 & 0.175 & 0.210 & 0.207 & 0.138 & 0.166 \\
    \multirow{1}{*}{GPT-4}  & 0.504 & 0.527 & 0.515 & - & - & - & - & - & - \\
    \multirow{1}{*}{LLaMa2-13B}  & 0.347 & 0.340 & 0.344 & 0.386 & 0.225 & 0.284 & 0.374 & 0.215 & 0.273 \\
    \multirow{1}{*}{Zephyr-7B-$\beta$}  & 0.214 & 0.229 & 0.221 & 0.192 & 0.180 & 0.185 & 0.148 & 0.142 & 0.145 \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:alignment_extraction}
\end{table}

\begin{table}[t]
    \centering
        \caption{Alignment results (macro-average) on the taxonomy discovery task in the \texttt{en} vs \texttt{gib} setting.}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cp{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}}
    \toprule
         \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{WN-sweets}} & \multicolumn{3}{c}{\textbf{WN-football}} & \multicolumn{3}{c}{\textbf{WN-music}}  \\
         \cline{2-10}
         & Pre. & Rec. & F1 & Pre. & Rec. & F1 & Pre. & Rec. & F1\\
    \midrule
    \multirow{1}{*}{GPT-3.5}  & 0.789 & 0.541 & 0.465 & 0.700 & 0.517 & 0.488 & 0.738 & 0.544 & 0.459 \\
    \multirow{1}{*}{GPT-4}  & 0.611 & 0.594 & 0.590 & - & - & - & - & - & - \\
    \multirow{1}{*}{LLaMa2-13B}  & 0.565 & 0.570 & 0.556 & 0.618 & 0.610 & 0.586 & 0.641 & 0.599 & 0.535 \\
    \multirow{1}{*}{Zephyr-7B-$\beta$}  & 0.818 & 0.727 & 0.716 & 0.557 & 0.544 & 0.545 & 0.570 & 0.572 & 0.570 \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:alignment_discovery}
\end{table}

\begin{comment}
\begin{table}[t]
\centering
\caption{F1-scores on different lexical semantic tasks in the GT(X) vs X setting, where X is either Real or Fake. In the taxonomy discovery task, * indicates that the F1-score for the positive class is extremely low (0.05 or less).}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Model} & \multicolumn{3}{c|}{relation extraction (F1)} & \multicolumn{3}{c|}{taxonomy discovery (Macro-avg. F1)} \\
\cline{2-7}
 & WN-sweets & WN-football & WN-music & WN-sweets & WN-football & WN-music \\
\hline
GPT-3.5 & 0.23 $\rightarrow$ 0.12 & 0.10 $\rightarrow$ 0.07  & & 0.57 $\rightarrow$ 0.35* & 0.52 $\rightarrow$ 0.29* & $\rightarrow$ \\
GPT-4 & & & & & & \\
LLaMa2-13B & 0.22 $\rightarrow$ 0.14 & 0.10$\rightarrow$ 0.08  & & 0.75 $\rightarrow$ 0.61  &  & $\rightarrow$ \\
Zephyr-7B-$\beta$ & 0.22 $\rightarrow$ 0.14 & & & 0.90 $\rightarrow$ 0.62 & $\rightarrow$ & $\rightarrow$  \\
\hline
\end{tabular}
\label{tab:model_performance}
\end{table}
\begin{table}[t]
\centering
\caption{Alignment F1-scores on different lexical semantic tasks in the Real vs Fake setting. * indicates that the F1-score for the positive class is extremely low (0.1 or less).}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Model} & \multicolumn{3}{c|}{relation extraction (F1)} & \multicolumn{3}{c|}{taxonomy discovery (Macro-avg. F1)} \\
\cline{2-7}
 & WN-sweets & WN-football & WN-music & WN-sweets & WN-football & WN-music \\
\hline
GPT-3.5 & 0.371 & 0.22 & & 0.51* & & \\
GPT-4 & & & & & & \\
LLaMa2-13B & 0.40 & 0.38 & & & & \\
Zephyr-7B-$\beta$ & 0.27 & & & 0.70 & & \\
\hline
\end{tabular}
\label{tab:model_alignment}
\end{table}
\end{comment}

\subsubsection{Results.} We first examine the results with respect the to ground-truths.
To preface this part, it is important to mention that the English WordNet is scarcely annotated in terms of hypernymy and holonymy relationships. Consider:
\begin{mdframed}
\begin{example}[toffee apple]
    an apple that is covered with a candy-like substance (usually caramelized sugar).
\label{toffee_apple}
\end{example}
\end{mdframed}

In Example~\ref{toffee_apple}, the definition obviously implies that a \textit{toffee apple} is an \textit{apple}, but WordNet only considers \textit{sweet, confection} to be valid hypernyms. The incompleteness of WordNet explains why the observed performances are so low, but because our goal is to compare performances using real corpora and their gibberish counterpart, it is not essential to have a high-quality ground-truth.

In both tasks, the results of which are reported in Table~\ref{tab:gt_rel_extraction_results} and Table~\ref{tab:gt_tax_disc_results}, a common trend occurs across all LLMs and in all synthetic domains: a significant performance decrease is observed when replacing real terms with gibberish. Although GPT-4 (tested on WN-sweets only because of the slowness and the costs) performs best on gibberish corpora, it suffers from the same performance drop.

While the performance on the relation extraction task is generally low across all models with the real datasets, which we mainly attribute to the poor quality of the annotations, it is even lower when using the gibberish datasets. In each case, the macro F1-score is practically halved, e.g. in the sweets domain, GPT-3.5 drops from 0.228 to 0.115, LLaMa2-13B drops from 0.223 to 0.138, Zephyr-7B-$\beta$ drops from 0.233 to 0.137. However, note that the recall is low in comparison to the precision, which indicates that a LLM already tends to overlook indicators that two concepts are hierarchically related. This observation aligns with the conclusion of LLMs4OL~\cite{giglou2023llms4ol}, according to which off-the-shelf LLMs are not sufficiently suitable for OL tasks, particularly in the case of relation extraction.

In the taxonomy discovery task where a classification prompt is used, the performance of large language models plummets when using the gibberish dataset instead of the real one. The LLMs are relatively good at identifying whether two real concepts are hierarchically related (F1-score up to 0.940 on the WN-sweets dataset by GPT-3.5), but suffer from a large performance drop when confronted to unknown words which share the same semantic relations (the F1-score of GPT-3.5 drops from 0.940 to 0.446 when using the gibberish counterpart of WN-sweets; the same behavior is observed across all datasets and LLMs). We interpret this drop as the fact that LLMs are significantly better at leveraging semantic priors, to deduce that Concept A is a subclass of Concept B.

Although the general performance drop is expected because the tested LLM would then be dealing with words it has never seen during its training, we furthermore observe that the prediction alignment is very low. In spite of analogous concepts sharing the same semantic relations with each other in the parallel corpora, the model is unable to produce analogous outputs from analogous inputs, as shown by the low F1-scores in Tables~\ref{tab:alignment_extraction} and~\ref{tab:alignment_discovery}. This is evidence that as is, LLMs do not \textit{reason} over semantic relationships.

Our interpretation is that the attention mechanism heavily relies on the lexical sense and the frame of a token, instead of leveraging the semantic relationships that hold between tokens. In other words, the "reasoning" abilities of LLMs for Ontology Learning are mostly limited to entities and concepts that the models have already been trained on, i.e. prior semantics. However, such a quality is critical for Ontology Learning in arbitrary domains, where hypernymy relationships must be retrieved for unknown concepts, or new concepts that share the same lexical form as some existing word (for instance, if domain-specific jargon employs existing words with different meanings).

This trend seems to hold true in both tasks, which confirms the fact that off-the-shelf LLMs are currently not suited for OL tasks on arbitrary domains.

\subsection{Fine-Tuning Evaluation}

\begin{table}[t]
\centering
\caption{Hypernym train-test split for the fine-tuning experiment.}
\begin{tabular}{ccccc}
\toprule
\multirow{2}{*}{$\mathcal{D}$} & \multicolumn{2}{c}{\textbf{Train}} & \multicolumn{2}{c}{\textbf{Test}}\\
& Positives & Negatives & Positives & Negatives\\
\midrule
\textbf{WN-sweets} & 189 & 393 & 229 & 284\\
\textbf{WN-football} & 674 & 1043 & 727 & 567 \\
\textbf{WN-music} & 1367 & 1882 & 1130 & 851 \\
\bottomrule
\end{tabular}
\label{tab:split}
\end{table}

\subsubsection{Training details.} Table~\ref{tab:split} shows the number of hypernym pairs used for the fine-tuning experiment. We use instruction tuning specifically tailored towards taxonomy discovery. In the prefix prompt documented in Listing~\ref{prompts_train}, given two concepts $A$ and $B$, the model must return ``True" if $A$ is a subclass of $B$ and ``False" otherwise. We train the model on 20 epochs, with a batch size of $4$ and a learning rate of $3 \cdot 10^{-6} $. For efficient training, we quantize the model on 4 bits and use the LoRA~\cite{hu2021lora} method with parameters $\alpha = 256$ and $r = 1024$.

\subsubsection{Metrics.} Similarly to the first experiment, we use Precision, Recall and F1-score to evaluate the performance of the model on the testing set.

\begin{table}[t]
    \centering
    \caption{Taxonomy discovery results with fine-tuning in the GT(X) vs X setting, where X is either \texttt{en} or \texttt{gib}. Evaluation is performed before and after fine-tuning.}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cp{1.cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}}
    \toprule
         \multirow{2}{*}{\textbf{Model (X)}} & \multirow{2}{*}{\textbf{When}} & \multicolumn{3}{c}{\textbf{WN-sweets}} & \multicolumn{3}{c}{\textbf{WN-football}} & \multicolumn{3}{c}{\textbf{WN-music}}  \\
         \cline{3-11}
         & & Pre. & Rec. & F1 & Pre. & Rec. & F1 & Pre. & Rec. & F1\\
    \midrule
    \multirow{2}{*}{Falcon-7B (\texttt{en})} & Before & 0.564 & 0.507 & 0.388 & 0.561 & 0.504 & 0.325 & 0.631 & 0.509 & 0.327 \\
         & After &  0.923 & 0.902 & 0.907 & 0.867 & 0.871 & 0.868 & 0.874 & 0.881 & 0.874 \\
         \midrule
    \multirow{2}{*}{Falcon-7B (\texttt{gib})} & Before & 0.275& 0.491 & 0.352 & 0.594 & 0.501 & 0.309 & 0.314 & 0.498 & 0.300 \\
         & After & 0.725 & 0.663 & 0.655 & 0.685 & 0.687 & 0.679 & 0.708 & 0.703 & 0.683 \\
         \midrule
    \multirow{2}{*}{Zephyr-7B-$\beta$ (\texttt{en})} & Before & 0.898 & 0.845 & 0.853 & 0.772 & 0.679 & 0.618 & 0.783 & 0.722 & 0.674 \\
         & After & 0.905 & 0.906 & 0.897 & 0.940 & 0.939 & 0.939 & 0.941 & 0.939 & 0.940 \\
         \midrule
    \multirow{2}{*}{Zephyr-7B-$\beta$ (\texttt{gib})} & Before & 0.746 & 0.572 & 0.500 & 0.740 & 0.621 & 0.535 & 0.723 & 0.589 & 0.479 \\
         & After & 0.840 & 0.816 & 0.796 & 0.859 & 0.810 & 0.817 & 0.839 & 0.846 & 0.839 \\
         \midrule
    \end{tabular}
    }
    \label{tab:finetuning_exp_res}
\end{table}

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{images/results_transfer_zephyr.pdf}
    \caption{Domain transfer experiment results with Zephyr-7B-$\beta$. Only gibberish corpora are selected for both training and testing.}
    \label{fig:transfer_results}
    % \vspace{-0.4cm}
\end{figure}

\subsubsection{Results.} The results of the fine-tuning experiment are reported in Table~\ref{tab:finetuning_exp_res}. Two general observations can be made about the experiment.
Firstly, we notice that fine-tuning drastically improves the task-specific performance of the LLM regardless the domain and corpus version. For instance, while Falcon-7B seems to be initially worse-performing than Zephyr-7B-$\beta$ overall, the F1-score improves up to almost threefold (real WN-music dataset, from 0.327 to 0.874). Although not surprising for real corpora, an improvement on gibberish corpora is nontrivial: the LLMs show signs of adaptation on gibberish corpora with improved performance. Secondly, while the performance of a model on a gibberish corpus increases after fine-tuning, it never matches the performance of the same model fine-tuned on the real counterpart of the corpus. It is worth noting that this is a limitation of adaptation solely due to the reliance on prior semantics, since a corpus and its gibberish counterpart only differ in their input-label mapping.

\subsubsection{Transfer Learning.} In spite of the two previous observations, we can hypothesize that the improvement in performance on the gibberish corpora may indicate signs of reasoning and generalization on unseen domains, given that gibberish words are most likely not contained in the vocabulary of LLMs. To elaborate this claim, we propose another experiment: we use Zephyr-7B-$\beta$, trained for taxonomy discovery in a domain, and test it on another domain. By only using gibberish corpora, we ensure that most of the domain-specific terminology is anonymized, preventing the LLM from effectively using prior semantics. Results are reported in Figure~\ref{fig:transfer_results}. We observe the following. Firstly, the F1-scores generally tend to increase after transfer, with the exception of the WN-music to WN-sweets case. The increase in F1-score is substantial, from 14\% (WN-football to WN-sweets), up to 32\% (WN-music to WN-football). This result is quite promising, as it points towards the possibility of OL on arbitrary domains with LLMs with effective pre-training. Secondly, the precision tends to drop in favor of the recall, indicating that fine-tuning makes the LLM more sensitive to syntactic clues of hypernymy relations at the cost of making them less precise. Due to the fact that both the training and the testing domains are made of gibberish words, we attribute the performance improvements of the LLM (with respect to its base version) to emerging reasoning capabilities: the fine-tuning LLM becomes more capable of abstraction and of focusing on semantic relationships between concepts, rather than the concepts themselves.

==> sections/experiments/finetuning_falcon.tex <==
batch_size=4, gradient_accumulation_steps=2, learning_rate=3e-06, logging_steps=1, num_train_epochs=20, max_steps=-1, log_with=None, save_steps=100, save_total_limit=10, lora_r=1024, lora_alpha=256


================ FOOTBALL ======================
REAL

[INFO] Evaluating on Train split
              precision    recall  f1-score   support

           0      0.608     0.982     0.751      1043
           1      0.424     0.021     0.040       674

    accuracy                          0.605      1717
   macro avg      0.516     0.501     0.395      1717
weighted avg      0.536     0.605     0.472      1717

[INFO] Evaluating on Test split
              precision    recall  f1-score   support

           0      0.440     0.988     0.609       567
           1      0.682     0.021     0.040       727

    accuracy                          0.444      1294
   macro avg      0.561     0.504     0.325      1294
weighted avg      0.576     0.444     0.289      1294

[INFO] Final Evaluation on Train split
              precision    recall  f1-score   support

           0      0.941     0.937     0.939      1043
           1      0.903     0.909     0.906       674

    accuracy                          0.926      1717
   macro avg      0.922     0.923     0.923      1717
weighted avg      0.926     0.926     0.926      1717

[INFO] Final Evaluation on Test split
              precision    recall  f1-score   support

           0      0.828     0.885     0.856       567
           1      0.906     0.857     0.881       727

    accuracy                          0.869      1294
   macro avg      0.867     0.871     0.868      1294
weighted avg      0.872     0.869     0.870      1294


GIBBERISH

[INFO] Evaluating on Train split
              precision    recall  f1-score   support

           0      0.609     1.000     0.757      1043
           1      1.000     0.006     0.012       674

    accuracy                          0.610      1717
   macro avg      0.804     0.503     0.384      1717
weighted avg      0.762     0.610     0.464      1717

[INFO] Evaluating on Test split
              precision    recall  f1-score   support

           0      0.439     0.998     0.610       567
           1      0.750     0.004     0.008       727

    accuracy                          0.440      1294
   macro avg      0.594     0.501     0.309      1294
weighted avg      0.614     0.440     0.272      1294

[INFO] Final Evaluation on Train split
              precision    recall  f1-score   support

           0      0.796     0.884     0.838      1043
           1      0.784     0.650     0.710       674

    accuracy                          0.792      1717
   macro avg      0.790     0.767     0.774      1717
weighted avg      0.791     0.792     0.788      1717

[INFO] Final Evaluation on Test split
              precision    recall  f1-score   support

           0      0.609     0.750     0.672       567
           1      0.762     0.624     0.686       727

    accuracy                          0.679      1294
   macro avg      0.685     0.687     0.679      1294
weighted avg      0.695     0.679     0.680      1294


================ SWEETS ========================

REAL

[INFO] Evaluating on Train split
              precision    recall  f1-score   support

           0      0.674     0.972     0.796       393
           1      0.267     0.021     0.039       189

    accuracy                          0.663       582
   macro avg      0.470     0.497     0.418       582
weighted avg      0.542     0.663     0.550       582

[INFO] Evaluating on Test split
              precision    recall  f1-score   support

           0      0.557     0.979     0.710       284
           1      0.571     0.035     0.066       229

    accuracy                          0.558       513
   macro avg      0.564     0.507     0.388       513
weighted avg      0.564     0.558     0.423       513

[INFO] Final Evaluation on Train split
              precision    recall  f1-score   support

           0      0.937     0.944     0.940       393
           1      0.882     0.868     0.875       189

    accuracy                          0.919       582
   macro avg      0.909     0.906     0.908       582
weighted avg      0.919     0.919     0.919       582

[INFO] Final Evaluation on Test split
              precision    recall  f1-score   support

           0      0.872     0.982     0.924       284
           1      0.974     0.821     0.891       229

    accuracy                          0.910       513
   macro avg      0.923     0.902     0.907       513
weighted avg      0.918     0.910     0.909       513


GIBBERISH

[INFO] Evaluating on Train split
              precision    recall  f1-score   support

           0      0.676     0.995     0.805       393
           1      0.500     0.011     0.021       189

    accuracy                          0.675       582
   macro avg      0.588     0.503     0.413       582
weighted avg      0.619     0.675     0.551       582

[INFO] Evaluating on Test split
              precision    recall  f1-score   support

           0      0.549     0.982     0.705       284
           1      0.000     0.000     0.000       229

    accuracy                          0.544       513
   macro avg      0.275     0.491     0.352       513
weighted avg      0.304     0.544     0.390       513

[INFO] Final Evaluation on Train split
              precision    recall  f1-score   support

           0      0.737     0.804     0.769       393
           1      0.497     0.402     0.444       189

    accuracy                          0.674       582
   macro avg      0.617     0.603     0.607       582
weighted avg      0.659     0.674     0.664       582

[INFO] Final Evaluation on Test split
              precision    recall  f1-score   support

           0      0.659     0.912     0.765       284
           1      0.792     0.415     0.544       229

    accuracy                          0.690       513
   macro avg      0.725     0.663     0.655       513
weighted avg      0.718     0.690     0.667       513

=========== MUSIC ========================

Number of train positives : 1367
Number of train negatives : 1882
Number of test positives : 1130
Number of test negatives : 851

REAL
[INFO] Evaluating on Train split
              precision    recall  f1-score   support

           0      0.580     0.967     0.725      1882
           1      0.447     0.037     0.069      1367

    accuracy                          0.576      3249
   macro avg      0.514     0.502     0.397      3249
weighted avg      0.524     0.576     0.449      3249

[INFO] Evaluating on Test split
              precision    recall  f1-score   support

           0      0.434     0.993     0.604       851
           1      0.829     0.026     0.050      1130

    accuracy                          0.441      1981
   macro avg      0.631     0.509     0.327      1981
weighted avg      0.659     0.441     0.288      1981

[INFO] Final Evaluation on Train split
              precision    recall  f1-score   support

           0      0.979     0.973     0.976      1882
           1      0.964     0.971     0.967      1367

    accuracy                          0.972      3249
   macro avg      0.971     0.972     0.972      3249
weighted avg      0.972     0.972     0.972      3249

[INFO] Final Evaluation on Test split
              precision    recall  f1-score   support

           0      0.815     0.919     0.864       851
           1      0.932     0.842     0.885      1130

    accuracy                          0.875      1981
   macro avg      0.874     0.881     0.874      1981
weighted avg      0.882     0.875     0.876      1981


GIBBERISH

[INFO] Evaluating on Train split
              precision    recall  f1-score   support

           0      0.580     1.000     0.734      1882
           1      1.000     0.002     0.004      1367

    accuracy                          0.580      3249
   macro avg      0.790     0.501     0.369      3249
weighted avg      0.757     0.580     0.427      3249

[INFO] Evaluating on Test split
              precision    recall  f1-score   support

           0      0.429     0.995     0.599       851
           1      0.200     0.001     0.002      1130

    accuracy                          0.428      1981
   macro avg      0.314     0.498     0.300      1981
weighted avg      0.298     0.428     0.258      1981

[INFO] Final Evaluation on Train split
              precision    recall  f1-score   support

           0      0.895     0.903     0.899      1882
           1      0.865     0.854     0.859      1367

    accuracy                          0.882      3249
   macro avg      0.880     0.879     0.879      3249
weighted avg      0.882     0.882     0.882      3249

[INFO] Final Evaluation on Test split
              precision    recall  f1-score   support

           0      0.593     0.838     0.695       851
           1      0.823     0.567     0.672      1130

    accuracy                          0.683      1981
   macro avg      0.708     0.703     0.683      1981
weighted avg      0.724     0.683     0.681      1981

==> sections/experiments/finetuning_zephyr.tex <==
ZEPHYR

================ SWEETS ======================
Number of train positives : 189
Number of train negatives : 393
Number of test positives : 229
Number of test negatives : 284

REAL
[INFO] Evaluating on Train split
              precision    recall  f1-score   support

           0      0.797     0.990     0.883       393
           1      0.957     0.476     0.636       189

    accuracy                          0.823       582
   macro avg      0.877     0.733     0.760       582
weighted avg      0.849     0.823     0.803       582

[INFO] Evaluating on Test split
              precision    recall  f1-score   support

           0      0.802     0.996     0.889       284
           1      0.994     0.694     0.817       229

    accuracy                          0.862       513
   macro avg      0.898     0.845     0.853       513
weighted avg      0.887     0.862     0.857       513

[INFO] Final Evaluation on Train split
              precision    recall  f1-score   support

           0      1.000     0.847     0.917       393
           1      0.759     1.000     0.863       189

    accuracy                          0.897       582
   macro avg      0.880     0.924     0.890       582
weighted avg      0.922     0.897     0.900       582

[INFO] Final Evaluation on Test split
              precision    recall  f1-score   support

           0      0.996     0.817     0.897       284
           1      0.814     0.996     0.896       229

    accuracy                          0.897       513
   macro avg      0.905     0.906     0.897       513
weighted avg      0.915     0.897     0.897       513

GIBBERISH

[INFO] Evaluating on Train split
              precision    recall  f1-score   support

           0      0.705     0.985     0.822       393
           1      0.818     0.143     0.243       189

    accuracy                          0.711       582
   macro avg      0.762     0.564     0.532       582
weighted avg      0.742     0.711     0.634       582

[INFO] Evaluating on Test split
              precision    recall  f1-score   support

           0      0.592     0.986     0.740       284
           1      0.900     0.157     0.268       229

    accuracy                          0.616       513
   macro avg      0.746     0.572     0.504       513
weighted avg      0.729     0.616     0.529       513

[INFO] Final Evaluation on Train split
              precision    recall  f1-score   support

           0      1.000     0.494     0.661       393
           1      0.487     1.000     0.655       189

    accuracy                          0.658       582
   macro avg      0.744     0.747     0.658       582
weighted avg      0.833     0.658     0.659       582

[INFO] Final Evaluation on Test split
              precision    recall  f1-score   support

           0      0.989     0.641     0.778       284
           1      0.690     0.991     0.814       229

    accuracy                          0.797       513
   macro avg      0.840     0.816     0.796       513
weighted avg      0.856     0.797     0.794       513

================ FOOTBALL ======================

Number of train positives : 674
Number of train negatives : 1043
Number of test positives : 727
Number of test negatives : 567

REAL
[INFO] Evaluating on Train split
              precision    recall  f1-score   support

           0      0.688     0.990     0.812      1043
           1      0.953     0.304     0.461       674

    accuracy                          0.721      1717
   macro avg      0.821     0.647     0.636      1717
weighted avg      0.792     0.721     0.674      1717

[INFO] Evaluating on Test split
              precision    recall  f1-score   support

           0      0.548     0.998     0.708       567
           1      0.996     0.359     0.528       727

    accuracy                          0.639      1294
   macro avg      0.772     0.679     0.618      1294
weighted avg      0.800     0.639     0.607      1294

[INFO] Final Evaluation on Train split
              precision    recall  f1-score   support

           0      0.998     0.963     0.980      1043
           1      0.945     0.997     0.970       674

    accuracy                          0.976      1717
   macro avg      0.972     0.980     0.975      1717
weighted avg      0.977     0.976     0.976      1717

[INFO] Final Evaluation on Test split
              precision    recall  f1-score   support

           0      0.938     0.926     0.932       567
           1      0.943     0.952     0.947       727

    accuracy                          0.940      1294
   macro avg      0.940     0.939     0.939      1294
weighted avg      0.940     0.940     0.940      1294


GIBBERISH

[INFO] Evaluating on Train split
              precision    recall  f1-score   support

           0      0.651     0.979     0.782      1043
           1      0.852     0.188     0.309       674

    accuracy                          0.669      1717
   macro avg      0.752     0.584     0.545      1717
weighted avg      0.730     0.669     0.596      1717

[INFO] Evaluating on Test split
              precision    recall  f1-score   support

           0      0.508     0.991     0.671       567
           1      0.973     0.250     0.398       727

    accuracy                          0.575      1294
   macro avg      0.740     0.621     0.535      1294
weighted avg      0.769     0.575     0.518      1294

[INFO] Final Evaluation on Train split
              precision    recall  f1-score   support

           0      0.994     0.752     0.856      1043
           1      0.721     0.993     0.835       674

    accuracy                          0.846      1717
   macro avg      0.857     0.872     0.846      1717
weighted avg      0.887     0.846     0.848      1717

[INFO] Final Evaluation on Test split
              precision    recall  f1-score   support

           0      0.935     0.656     0.771       567
           1      0.782     0.964     0.864       727

    accuracy                          0.829      1294
   macro avg      0.859     0.810     0.817      1294
weighted avg      0.849     0.829     0.823      1294

======= MUSIC =====================

Number of train positives : 1367
Number of train negatives : 1882
Number of test positives : 1130
Number of test negatives : 851

[INFO] Evaluating on Train split
              precision    recall  f1-score   support

           0      0.712     0.990     0.828      1882
           1      0.971     0.448     0.614      1367

    accuracy                          0.762      3249
   macro avg      0.842     0.719     0.721      3249
weighted avg      0.821     0.762     0.738      3249

[INFO] Evaluating on Test split
              precision    recall  f1-score   support

           0      0.576     0.994     0.730       851
           1      0.990     0.450     0.618      1130

    accuracy                          0.683      1981
   macro avg      0.783     0.722     0.674      1981
weighted avg      0.812     0.683     0.666      1981

              precision    recall  f1-score   support

           0      0.987     0.955     0.971      1882
           1      0.941     0.982     0.961      1367

    accuracy                          0.967      3249
   macro avg      0.964     0.969     0.966      3249
weighted avg      0.968     0.967     0.967      3249

[INFO] Final Evaluation on Test split
              precision    recall  f1-score   support

           0      0.938     0.924     0.931       851
           1      0.943     0.954     0.949      1130

    accuracy                          0.941      1981
   macro avg      0.941     0.939     0.940      1981
weighted avg      0.941     0.941     0.941      1981


GIBBERISH

[INFO] Evaluating on Train split
              precision    recall  f1-score   support

           0      0.600     0.967     0.741      1882
           1      0.712     0.114     0.197      1367

    accuracy                          0.608      3249
   macro avg      0.656     0.540     0.469      3249
weighted avg      0.647     0.608     0.512      3249

[INFO] Evaluating on Test split
              precision    recall  f1-score   support

           0      0.478     0.992     0.646       851
           1      0.968     0.186     0.312      1130

    accuracy                          0.532      1981
   macro avg      0.723     0.589     0.479      1981
weighted avg      0.758     0.532     0.455      1981

[INFO] Final Evaluation on Train split
              precision    recall  f1-score   support

           0      0.967     0.979     0.973      1882
           1      0.970     0.954     0.962      1367

    accuracy                          0.968      3249
   macro avg      0.969     0.966     0.967      3249
weighted avg      0.968     0.968     0.968      3249

[INFO] Final Evaluation on Test split
              precision    recall  f1-score   support

           0      0.772     0.890     0.826       851
           1      0.906     0.802     0.851      1130

    accuracy                          0.839      1981
   macro avg      0.839     0.846     0.839      1981
weighted avg      0.848     0.839     0.840      1981

==> sections/experiments/transfer_zephyr.tex <==
OFF-THE-SHELF (Test on WN-sweets(gibberish))
              precision    recall  f1-score   support

           0      0.592     0.986     0.740       284
           1      0.900     0.157     0.268       229

    accuracy                          0.616       513
   macro avg      0.746     0.572     0.504       513
weighted avg      0.729     0.616     0.529       513

SWEETS(R) TO SWEETS(G)

Number of train positives : 189
Number of train negatives : 393
Number of test positives : 229
Number of test negatives : 284

AFTER TRAIN
              precision    recall  f1-score   support

           0      0.704     0.813     0.755       284
           1      0.714     0.576     0.638       229

    accuracy                          0.708       513
   macro avg      0.709     0.695     0.696       513
weighted avg      0.708     0.708     0.703       513

FOOTBALL(R) TO SWEETS(G)

              precision    recall  f1-score   support

           0      0.630     0.972     0.765       284
           1      0.893     0.293     0.441       229

    accuracy                          0.669       513
   macro avg      0.762     0.632     0.603       513
weighted avg      0.748     0.669     0.620       513


===================================================
FOOTBALL TO SWEETS

   macro avg      0.612     0.601     0.578       513
   
FOOTBALL TO MUSIC

   macro avg      0.627     0.627     0.627      1981

MUSIC TO SWEETS

   macro avg      0.512     0.508     0.475       513

MUSIC TO FOOTBALL

   macro avg      0.754     0.732     0.706      1294

SWEETS TO FOOTBALL

   macro avg      0.720     0.664     0.658      1294

SWEETS TO MUSIC
   macro avg      0.715     0.638     0.626      1981



==> sections/experiments/wn_sweets.tex <==
GPT3.5 :

Average F1 per sample : 0.3009912078662078
Overall F1 : 0.376429199648197

Real dataset vs ground-truth
              precision    recall  f1-score   support

           0       0.60      1.00      0.75       488
           1       0.98      0.24      0.38       418

    accuracy                           0.65       906
   macro avg       0.79      0.62      0.57       906
weighted avg       0.78      0.65      0.58       906

Gibberish dataset vs ground-truth
              precision    recall  f1-score   support

           0       0.54      1.00      0.70       488
           1       0.00      0.00      0.00       418

    accuracy                           0.54       906
   macro avg       0.27      0.50      0.35       906
weighted avg       0.29      0.54      0.38       906


LLaMa ("meta-llama/Llama-2-13b-chat-hf")
Average F1 per sample : 0.37891436409954926
Overall F1 : 0.39963996399639967

Real dataset vs ground-truth
              precision    recall  f1-score   support

           0       0.98      0.56      0.71       488
           1       0.66      0.99      0.79       418

    accuracy                           0.76       906
   macro avg       0.82      0.77      0.75       906
weighted avg       0.83      0.76      0.75       906

Gibberish dataset vs ground-truth
              precision    recall  f1-score   support

          -1       0.00      0.00      0.00         0
           0       0.81      0.39      0.53       488
           1       0.56      0.89      0.69       418

    accuracy                           0.62       906
   macro avg       0.46      0.43      0.40       906
weighted avg       0.69      0.62      0.60       906








